Bridging the Silos of Digitalization and Sustainability by Twin Transition: A Multivocal Literature Review

Twin transition is the method of parallel digital and sustainability transitions in a mutually supporting way or, in common terms, "greening of and by IT and data." Twin transition reacts to the growing problem of unsustainable digitalization, particularly in the ecological sense. Ignoring this problem will eventually limit the digital adeptness of society and the problem-solving capacity of humankind. Information systems engineering must find ways to support twin transition journeys through its substantial body of knowledge, methods, and techniques. To this end, we systematically survey the academic and gray literature on twin transition, clarify key concepts, and derive leads for researchers and practitioners to steer their innovation efforts.

==> tables/rq2-problems.tex <==
\begin{table}[tbh]
\scriptsize
\centering
\caption{Problems and motivations}
\label{tab:results-rq2-problems}
\begin{tabular}{@{}lll@{}}
\toprule
\multicolumn{1}{c}{\textbf{Motivation/problem}} & \multicolumn{1}{c}{\textbf{\#Studies}} & \multicolumn{1}{c}{\textbf{Studies}} \\ \midrule

\textbf{Policy and governance} & \maindatabar{11} & \\
\subcategory{} Policy ineffectiveness and consistency & \subdatabar{7} &\cite{brueck2024chinas, celeste2023digital, gao2024eus, kovacic2024twin, pan2024policy, poscic2024role, sanchez2024european} \\
\subcategory{} Competitiveness of companies & \subdatabar{3} &\cite{gigauri2023digital,myyrylainen2023small,rehman2023twin} \\
\subcategory{} Regional inequalities & \subdatabar{1} &\cite{bianchini2023environmental} \\

\textbf{Technology} & \maindatabar{8} & \\
\subcategory{} Eco-footprint of specific technology & \subdatabar{6} & \cite{balanici2023f5g, baum2024will, chen2023enabling, matinmikko-blue2021sustainability, niet2024framing, stucki2024data} \\
\subcategory{} Technology decarbonization & \subdatabar{1} & \cite{muller2023digitisation} \\
\subcategory{} IS for circular economy & \subdatabar{1} & \cite{reich2024towards} \\

\textbf{Sustainability fundamentals} & \maindatabar{6} & \\
\subcategory{} Informing (potential) end-users & \subdatabar{2} & \cite{korucuk2022assessing, tekavc2023pilot} \\
\subcategory{} Low leverage points of digital innovations & \subdatabar{2} & \cite{chen2023enabling,makitie2023digital} \\
\subcategory{} Dealing with techno-optimism & \subdatabar{1} & \cite{meijer2024perspectives} \\
\subcategory{} Ensuring sustainable consumption & \subdatabar{1} & \cite{chiu2020can} \\


\bottomrule
\end{tabular}
\end{table}

\iffalse
\begin{table}[tbh]
\scriptsize
\centering
\caption{Problems and motivations}
\label{tab:results-rq2-problems}
\begin{tabular}{@{}lll@{}}
\toprule
\multicolumn{1}{c}{\textbf{Motivation/problem}} & \multicolumn{1}{c}{\textbf{\#Studies}} & \multicolumn{1}{c}{\textbf{Studies}} \\ \midrule

\textbf{Policy and governance} & \maindatabar{11} & \\
\subcategory{} Policy effectiveness & \subdatabar{4} &\cite{brueck2024chinas, celeste2023digital, pan2024policy, poscic2024role} \\
\subcategory{} Policy consistency/ambiguity & \subdatabar{3} &\cite{gao2024eus, kovacic2024twin, sanchez2024european} \\
\subcategory{} Competitiveness of companies & \subdatabar{3} &\cite{gigauri2023digital,myyrylainen2023small,rehman2023twin} \\
\subcategory{} Regional inequalities & \subdatabar{1} &\cite{bianchini2023environmental} \\

\textbf{Technology} & \maindatabar{8} & \\
\subcategory{} Eco-footprint of specific technology & \subdatabar{6} & \cite{balanici2023f5g, baum2024will, chen2023enabling, matinmikko-blue2021sustainability, niet2024framing, stucki2024data} \\
\subcategory{} Technology decarbonization & \subdatabar{1} & \cite{muller2023digitisation} \\
\subcategory{} IS for circular economy & \subdatabar{1} & \cite{reich2024towards} \\

\textbf{Sustainability fundamentals} & \maindatabar{6} & \\
\subcategory{} Informing (potential) end-users & \subdatabar{2} & \cite{korucuk2022assessing, tekavc2023pilot} \\
\subcategory{} Low leverage points of digital innovations & \subdatabar{2} & \cite{chen2023enabling,makitie2023digital} \\
\subcategory{} Dealing with techno-optimism & \subdatabar{1} & \cite{meijer2024perspectives} \\
\subcategory{} Ensuring sustainable consumption & \subdatabar{1} & \cite{chiu2020can} \\


\bottomrule
\end{tabular}
\end{table}

\fi

==> tables/rq2-sustainability-dimensions.tex <==
%\begin{table}[t]
%\scriptsize
%\centering
%\caption{Sustainability dimensions}
%\label{tab:results-rq2-sustainability-dimensions}
{\footnotesize
\begin{tabular}{@{}lll@{}}
\toprule
\multicolumn{1}{c}{\textbf{Sus. dimension}} & \multicolumn{1}{c}{\textbf{\#Studies}} & \multicolumn{1}{c}{\textbf{Studies}} \\ \midrule

Environmental & \maindatabar{26} & \cite{balanici2023f5g, baum2024will, bianchini2023environmental, brueck2024chinas, celeste2023digital, chen2023enabling, chiu2020can, gao2024eus, gigauri2023digital, herczeg2023how, korucuk2022assessing, kovacic2024twin,lazazzara2024digital, makitie2023digital, matinmikko-blue2021sustainability, meijer2024perspectives, muller2023digitisation, myyrylainen2023small, niet2024framing, pan2024policy, poscic2024role, rehman2023twin, reich2024towards, sanchez2024european, stucki2024data, tekavc2023pilot} \\

Social & \maindatabar{12} & \cite{lazazzara2024digital, makitie2023digital, matinmikko-blue2021sustainability, meijer2024perspectives, muller2023digitisation, myyrylainen2023small, niet2024framing, pan2024policy, poscic2024role, rehman2023twin, reich2024towards, sanchez2024european, stucki2024data, tekavc2023pilot} \\

Economic & \maindatabar{12} & \cite{lazazzara2024digital, makitie2023digital, matinmikko-blue2021sustainability, meijer2024perspectives, muller2023digitisation, myyrylainen2023small, niet2024framing, pan2024policy, poscic2024role, rehman2023twin, reich2024towards, sanchez2024european, stucki2024data, tekavc2023pilot} \\

\bottomrule
\end{tabular}}
%\end{table}


    
    
